Visual Question Decomposition on Multimodal Large Language Models

Question decomposition has emerged as an effective strategy for prompting Large Language Models (LLMs) to answer complex questions. However, while existing methods primarily focus on unimodal language models, the question decomposition capability of Multimodal Large Language Models (MLLMs) has yet to be explored. To this end, this paper explores visual question decomposition on MLLMs. Specifically, we introduce a systematic evaluation framework including a dataset and several evaluation criteria to assess the quality of the decomposed sub-questions, revealing that existing MLLMs struggle to produce high-quality sub-questions. To address this limitation, we propose a specific finetuning dataset, DecoVQA+, for enhancing the model's question decomposition capability. Aiming at enabling models to perform appropriate selective decomposition, we propose an efficient finetuning pipeline. The finetuning pipeline consists of our proposed dataset and a training objective for selective decomposition. Finetuned MLLMs demonstrate significant improvements in the quality of sub-questions and the policy of selective question decomposition. Additionally, the models also achieve higher accuracy with selective decomposition on VQA benchmark datasets.

==> tables/err.tex <==
\begin{table}[htbp]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lll}
        \toprule
        \textbf{Models} & {\textbf{Version}}& {\textbf{Number of errors}}\\
        \midrule
        
         \multirow{4}{*}{\textbf{MiniGPT-v2}}&finetuned by DecoVQA & 29\\
         &finetuned by DecoVQA & 1\\ % Assuming \up{(+xx)} was to indicate an increase, replace with your actual value
         &finetuned by DecoVQA+ & 0\\
         &finetuned by DecoVQA+ with combined loss & 0\\
        \noalign{\vskip 1ex}\cdashline{1-3}\noalign{\vskip 1ex}
         
         \multirow{4}{*}{\textbf{LLaVA-1.5}}&finetuned by DecoVQA & 52\\
         &finetuned by DecoVQA & 1\\
         &finetuned by DecoVQA+ & 0\\
         &finetuned by DecoVQA+ with combined loss & 2\\
        \bottomrule
    \end{tabular}
    }
    \caption{Comparison of error frequencies in sub-question generation across different models on the same dataset. Errors are defined as instances where the model either directly answers the question without generating the required sub-questions or produces irrelevant content, contrary to the prompt's instructions.}
    \label{tab:err}
\end{table}

